Cooperative Localisation of a GPS-Denied UAV in 3-Dimensional Space Using Direction of Arrival Measurements

This paper presents a novel approach for localising a GPS (Global Positioning System)-denied Unmanned Aerial Vehicle (UAV) with the aid of a GPS-equipped UAV in three-dimensional space. The GPS-equipped UAV makes discrete-time broadcasts of its global coordinates. The GPS-denied UAV simultaneously receives the broadcast and takes direction of arrival (DOA) measurements towards the origin of the broadcast in its local coordinate frame (obtained via an inertial navigation system (INS)). The aim is to determine the difference between the local and global frames, described by a rotation and a translation. In the noiseless case, global coordinates were recovered exactly by solving a system of linear equations. When DOA measurements are contaminated with noise, rank relaxed semidefinite programming (SDP) and the Orthogonal Procrustes algorithm are employed. Simulations are provided and factors affecting accuracy, such as noise levels and number of measurements, are explored.

==> parts/next.tex <==
\subsection{Scope for further refinement}

The estimation $\overline{R}$ has the potential to be further refined though the use of maximum likelihood estimation. This process consists of minimising the cumulative error between expected and measured bearing angles for a given estimation of $\bm{R_A^B}$ and $\bm{T_A^B}$. This is achieved by evaluating the gradient over the cost function of cumulative error, and running a gradient descent algorithm using partial derivatives corresponding to the 6 degrees of freedom in the problem.
